Fragility and Robustness in Mean-Payoff Adversarial Stackelberg Games

Two-player mean-payoff Stackelberg games are nonzero-sum infinite duration games played on a bi-weighted graph by Leader (Player 0) and Follower (Player 1). Such games are played sequentially: first, Leader announces her strategy, second, Follower chooses his best-response. If we cannot impose which best-response is chosen by Follower, we say that Follower, though strategic, is adversarial towards Leader. The maximal value that Leader can get in this nonzero-sum game is called the adversarial Stackelberg value (ASV) of the game. We study the robustness of strategies for Leader in these games against two types of deviations: (i) Modeling imprecision - the weights on the edges of the game arena may not be exactly correct, they may be delta-away from the right one. (ii) Sub-optimal response - Follower may play epsilon-optimal best-responses instead of perfect best-responses. First, we show that if the game is zero-sum then robustness is guaranteed while in the nonzero-sum case, optimal strategies for ASV are fragile. Second, we provide a solution concept to obtain strategies for Leader that are robust to both modeling imprecision, and as well as to the epsilon-optimal responses of Follower, and study several properties and algorithmic problems related to this solution concept.

==> ExistenceOfASVEpsilonWitnessForFMStrategy.tex <==
Given a mean-payoff game $\mathcal{G}$, we study the problem of computing $\asv_{\mathsf{FM}}(v)$ where $v$ is a vertex in $\mathcal{G}$. We start by describing the notion of witness for $\asv_{\mathsf{FM}}$.

\noindent\textbf{Regular Witness for $\asv_{\mathsf{FM}}$} A play $\pi$ in G is called a $(c',d)^{\epsilon}$-witness of $\asvgen_{\mathsf{FM}}^{\epsilon}(v) > c$ if it starts from $v$, and $(\mpinf_0(\pi), \mpinf_1(\pi)) = (c', d)$, where $c' > c$ and $\pi$ does not contain any $(c,d)^{\epsilon}$-bad vertex. 
A play $\pi$ is called an $\epsilon$-regular-witness of $\asvgen_{\mathsf{FM}}^{\epsilon}(v) > c$ if it is a $(c',d)^{\epsilon}$-witness of $\asvgen_{\mathsf{FM}}^{\epsilon}(v) > c$ for some $c',d$ and it can be expressed as $\pi = \pi_1 (\pi_2)^{\omega}$, where $\pi_1, \pi_2$ are plays in $\mathcal{G}$.

\mbcomment{Also explain the variation of why it is different from the iCalp paper}
\btrack{Note that in \cite{FGR20}, no regular witness has been studied.}
In fact, there, only infinite memory strategies have been considered for the threshold problem.

\begin{lemma}
\label{lemWitnessASVForFinStrat}
For all mean-payoff games $\mathcal{G}$, for all $\epsilon > 0$, for all vertices $v$ in $\mathcal{G}$, for all rational constants $c \in \mathbb{Q}$, we have that $\asvgen_{\mathsf{FM}}^{\epsilon}(v) > c$ if and only if there exists a play $\pi$ in $\mathcal{G}$ which is an $\epsilon$-regular-witness for $\asvgen_{\mathsf{FM}}^{\epsilon}(v) > c$.
\end{lemma}
\begin{proof}
	Let $\pi = \pi_1 (\pi_2)^{\omega}$, where $\pi_1, \pi_2$ are plays in $\mathcal{G}$.
	First we prove the right to left direction, i.e., we are given a  play $\pi = \pi_1 (\pi_2)^{\omega}$ in $\mathcal{G}$ such that  $(\mpinf_0(\pi), \mpinf_1(\pi)) = (c', d)$, for some $c', d \in \mathbb{R}$ and $c' > c$ and $\pi$ does not contain any $(c,d)^{\epsilon}$-bad vertex. We need to prove that $\asvgen_{\mathsf{FM}}^{\epsilon}(v) > c$.
	
	We do this by defining a strategy $\sigma_0$ for Player~0 such that:
	\begin{enumerate}
		\item $\forall h \leqslant \pi$, and $last(h)$ is a Player~0 vertex, $\sigma_0(h)$ follows $\pi$. This is a finite memory strategy.
		\item $\forall h \nleqslant \pi$, where there has been a deviation from $\pi$ by Player~1, we assume Player~0 switches to a strategy that we call \textit{punishing}. This strategy is defined as follows: In the subgame after history $h'$, where $last(h')$ is the first vertex at which Player~1 deviated from $\pi$, we know that Player~0 has a strategy to enforce the objective: $\mpinf_0(\pi) > c$ $\lor$ $ \mpinf_1(\pi) \leqslant d-\epsilon$. This is true because $\pi$ does not cross any $(c,d)^{\epsilon}$-bad vertex and because n-dimension mean-payoff games are determined. We show that this is a memoryless strategy in \myChapter 4.
		\item For all other histories $h$ Player~0 can behave arbitrarily as those histories are never reached when Player~0 plays as defined in point 1 and 2 above.
	\end{enumerate}
	
	Let us now establish that strategy $\sigma_0$ satisfies $\asvgen_{\mathsf{FM}}^{\epsilon}(\sigma_0)(v) > c$. Since $\mpinf_1(\pi) = d$, we have that $\sup\limits_{\sigma_1 \in \br(\sigma_0)} \mpinf_1(\outv(\sigma_0, \sigma_1) \geqslant d$. Now let us consider some strategy $\sigma_1 \in \br(\sigma_0)$. Clearly, $\pi' = \outv(\sigma_0, \sigma_1)$ is such that $\mpinf_1(\pi') > d-\epsilon$. If $\pi = \pi'$, we know that $\mpinf_0(\pi') > c$. If $\pi' \neq \pi$, then when $\pi'$ deviates from $\pi$, Player~0 employs a punishing strategy, thus making sure that $\mpinf_0(\pi') > c \lor \mpinf_1(\pi') \leqslant d - \epsilon$. But since $\sigma_1 \in \br(\sigma_0)$, we know that $\mpinf_1(\pi') > d - \epsilon$. Thus, it must be true that $\mpinf_0(\pi') > c$.
	
	Second, for the left to right direction of the proof, we are given that $\asvgen_{\mathsf{FM}}^{\epsilon}(v) > c$. This means that there is a finite memory strategy $\sigma_0$ for Player~0 such that $\asvgen_{\mathsf{FM}}^{\epsilon}(\sigma_0)(v) > c$. Let $d \in \mathbb{R}$ be the value such that:
	\begin{equation*}
	    d = \sup\limits_{\sigma_1 \in \br(\sigma_0)} \mpinf_1(\outv(\sigma_0, \sigma_1))
	\end{equation*}
	Let $\sigma_0$ be a finite memory strategy of size $M$. When Player~0 plays $\sigma_0$ on $\mathcal{G}$, we can construct a single player game for Player~1 of size $|\mathcal{G}|\times M$. We call this game $\mathcal{G}^M_{\sigma_0}$. In the game $\mathcal{G}^M_{\sigma_0}$, Player~1 has a memoryless strategy to obtain maximum mean-payoff value, i.e. the $\sup$ $d$ is reached. This memoryless strategy in $\mathcal{G}^M_{\sigma_0}$ can be translated to a finite memory strategy $\sigma_1$ in $\mathcal{G}$ such that $\mpinf_1(\outv(\sigma_0, \sigma_1)) = d$.
	Consider $\pi = \outv(\sigma_0, \sigma_1)$. Since both the players play finite memory strategies in $\pi$, we have that $\pi = \pi_1(\pi_2)^{\omega}$ where $\pi_1, \pi_2$ are finite plays. Consider some $\pi' \in \outv(\sigma_0))$. Clearly, if $\mpinf_1(\pi') > d-\epsilon$, then there exists a strategy $\sigma'_1 \in \br(\sigma_0)$ such that $\pi' = \outv(\sigma_0, \sigma'_1)$ and we conclude that $\mpinf_0(\pi') > c$. So all deviations of Player~1 w.r.t $\pi$ against $\sigma_0$ either give him $\mpinf_0(\pi') > c$ or $\mpinf_1(\pi') \leqslant d-\epsilon$. Thus, $\pi$ becomes a $\epsilon$-witness for $\asvgen_{\mathsf{FM}}^{\epsilon}(v) > c$ as it never crosses a $(c,d)^{\epsilon}$-bad vertex.
\end{proof}

==> FiniteMemForEpsASV.tex <==
\begin{lemma}
\label{LemFinMemWitnessASV}
For all mean-payoff games $\mathcal{G}$, for all vertices $v$ in $\mathcal{G}$, for all $\epsilon > 0$, and for all rationals $c$, if $\asv(v) > c$, then there exists a finite memory strategy $\sigma_0^v$ for Player~0 such that $\asv(\sigma_0^v)(v) > c$.
\end{lemma}

\begin{proof}
Given that $\asv(v) > c$, from \cref{LemPlaysAsWitnessForASV}, we know that there exists three acyclic finite plays $\pi_1, \pi_2, \pi_3$, and two simple cycles $l_1, l_2$ such that a play $\pi = \pi_1\rho_1\rho_2\rho_3\dots$ , where $\rho_i = l_1^{[\alpha i]}.\pi_2.l_2^{[\beta i]}.\pi_3$ for some $\alpha, \beta \in \mathbb{Q}^{+}$ and $\alpha + \beta = 1$. 
We call this play $\pi$ an  $\epsilon$-witness for $\asv(v) > c$.

Note that with $\pi$ we can construct an infinite memory strategy for Player~0 so as to minimise the effect of $\pi_2$ and $\pi_3$ on the mean-payoff measure, as specified in \cref{LemPlaysAsWitnessForASV}.
Let $\mpinf_0(\pi) = c'' > c$ and $\mpinf_1(\pi) = d$.

\noindent The mean-payoffs of the play $\pi$ are: $\mpinf_0(\pi) = \alpha \cdot w_0(l_1) + \beta \cdot w_0(l_2)$ and $\mpinf_1(\pi) = \alpha \cdot w_1(l_1) + \beta \cdot w_1(l_2)$. To obtain a finite memory strategy, we can modify the play $\pi$ as described below:
\begin{caseof}
    \case{$w_0(l_1) > w_0(l_2)$ and $w_1(l_1) < w_1(l_2)$}
    Here, one simple cycle, $l_1$, increases Player~0's mean-payoff while the other simple cycle, $l_2$, increases Player~1's mean-payoff. We can build a witness $\pi' = \pi_1.(l_1^{[\alpha]k}.\pi_2.l_2^{[\beta+\tau]k}.\pi_3)^{\omega}$ for some very large $k \in \mathbb{N}$ and for some very small $\tau > 0$ such that $\mpinf_0(\pi') > c$ and $\mpinf_1(\pi') = d$.\footnote{For more details, we refer the reader to the Appendix.}
    \case{$w_0(l_1) < w_0(l_2)$ and $w_1(l_1) > w_1(l_2)$}
    This is analogous to \textbf{case 1}, and proceeds as mentioned above.
    \case{$w_0(l_1) < w_0(l_2)$ and $w_1(l_1) < w_1(l_2)$}
    One cycle, $l_2$, increases both Player~0 and Player~1's mean-payoffs, while the other, $l_1$, decreases it. In this case, we can just omit one of the cycles - whichever cycle gives a larger mean-payoff, to get a finite memory strategy. Thus, $\pi' = \pi_1.l_2^{\omega}$ and we get $\mpinf_0(\pi') > c$ , $\mpinf_1(\pi') \geqslant d$.
    \case{$w_0(l_1) > w_0(l_2)$ and $w_1(l_1) > w_1(l_2)$}
    This is analogous to \textbf{case 3} and proceeds as mentioned above.
\end{caseof}
In each of these cases, we can show that $\pi'$ is a witness for $\asv(v) > c$: $\mpinf_0(\pi') > c$ and $\mpinf_1(\pi') \geqslant d$.
Since we know from \cref{LemPlaysAsWitnessForASV} that $\pi$ does not cross a $(c,d)^{\epsilon}$-bad vertex, the modified play $\pi'$ does not either, as the vertices of the play $\pi'$ are a subset of the vertices of the play $\pi$. 

Using $\pi'$, we build a finite memory strategy $\sigma_0^v$ for Player~0 as stated below:
\begin{enumerate}
    \item Player~0 follows $\pi'$ if Player~1 does not deviate from $\pi'$. The finite memory strategy stems from the finite $k$ as required in the four cases mentioned above.
    \item \label{strategy_memoryless} For each vertex $v \in \pi'$, Player~0 employs a memoryless strategy that establishes $v \nvDash \ll 1 \gg \mpinf_0 \leqslant c \land \mpinf_1 > d-\epsilon$.
\end{enumerate}
Thus, we see that $\asv(\sigma_0)(v) > c$.
The existence of the memoryless strategies mentioned in Point \ref{strategy_memoryless} above is established below. \\ \\ \noindent
The goal here is to obtain a memoryless strategy for Player~0 to achieve her objective, i.e., for all vertices $v \in \pi'$, ensure that $v \nvDash \ll 1 \gg \mpinf_0 \leqslant c \land \mpinf_1 > d-\epsilon$. \\ \noindent
We begin by constructing a game $\mathcal{G'}$ from the given game $\mathcal{G}$ by multiplying the first dimension on each edge of the game by $-1$. It is easy to see that, for all vertices $v \in \mathcal{G}$, we have that $v \nvDash \ll 1 \gg \mpinf_0 \leqslant c \land \mpinf_1 > d-\epsilon$ if and only if for the corresponding vertex in the game $\mathcal{G'}$, we have $v \nvDash \ll 1 \gg \overline{\mpgen}_0 \geqslant -c \land \mpinf_1 > d-\epsilon$.
From \cref{ConjGrtIsGrtEq}, we have $v \nvDash \ll 1 \gg \overline{\mpgen}_0 \geqslant -c \land \mpinf_1 \geqslant d'$, where $d' > d$.

We modify the game $\mathcal{G'}$ further by adding $c$ to the first dimension, and subtracting $d'$ from the second dimension for all the edges in the game. Note that the edges and vertices of both games $\mathcal{G}$ and $\mathcal{G'}$ are the same, the only difference between the two games being their edge weights. Thus, we get a modified objective for Player~0 in $\mathcal{G'}$, i.e., Player~0 wins if for all vertices $v \in \pi'$, we have that $v \nvDash \ll 1 \gg \overline{\mpgen}_0 \geqslant 0 \land \mpinf_1 \geqslant 0$.

Now the existence of a memoryless winning strategy for Player~0 follows from the result for Multi-weighted two-player games with $\mathbf{MeanPayoffInfSup}$ objective \cite{VCDHRR15} mentioned in \cref{ThmMemlessStrForP2}.

We formulate $\mathcal{G'}$ as a multi-weighted two-player game structure specified in \cref{ThmMemlessStrForP2} with $I = \{1\}$ and $J = \{0\}$. By \cref{ThmMemlessStrForP2}, we know that Player~0 has a memoryless winning strategy for all vertices $v \in \pi'$ in the game $\mathcal{G'}$ (since she wins for the same vertices in the game $\mathcal{G}$).
Thus, by \cref{PropGamStrEqNewGamStr}, for all vertices $v \in \pi'$, the finite memory strategy $\sigma_0^v$ is also winning for Player~0 in $\mathcal{G}$, that is, $\asv(\sigma_0)(v) > c$.
\end{proof}

Now, we establish that, in a mean-payoff game $\mathcal{G}$, the $\asv$ of a vertex $v$ in the game $\mathcal{G}$ does not change even if Player~0 is restricted to using only finite memory strategies. Formally, we state that:

\begin{corollary}
\label{CorASVEqASVFin}
In a mean-payoff game $\mathcal{G}$, if $\mathbf{ASV^{\epsilon}}(v) = c$, then for every $c' < c$, there exists a finite memory strategy $\sigma_0^{FM}$ for Player~0 which achieves $\mathbf{ASV^{\epsilon}}(\sigma_0^{FM})(v) > c'$. This implies that $\sup\limits_{\sigma_0 \in \Sigma_0^{\mathsf{FM}}} \mathbf{ASV^{\epsilon}}(\sigma_0)(v) = \mathbf{ASV^{\epsilon}}(v) = c$.
\end{corollary}

==> Introduction.tex <==

\noindent Stackelberg games \cite{S34} were first introduced to model strategic interactions among rational agents in markets that consist of a leader and followers.
The leader in the market makes her strategy public and the followers respond by playing an optimal response to this strategy.
Here, we consider Stackelberg games as a framework for the synthesis of reactive programs \cite{PR89,BCHPRRS16}.
These programs maintain a continuous interaction with the environment in which they operate; they are \emph{deterministic functions} that given a history of interactions so far choose an action.
Our work is a contribution to \emph{rational synthesis} \cite{FKL10,KPV16}, a nonzero-sum game setting where both the program and the environment are considered as rational agents that have their own goals.
While Boolean $\omega$-regular payoff functions have been studied in \cite{FKL10,KPV16}, here we study the quantitative long-run average (mean-payoff) function. 

We illustrate our setting with the example of a game graph shown in \cref{fig:robust-game-example}. 

The set $V$ of vertices is partitioned into $V_0$ (represented by circles) and $V_1$ (represented by squares) that are owned by the leader (also called Player~0) and the follower (also called Player~1) respectively.
In the tuple on the edges, the first one is the payoff of the leader, while the second one is the payoff of the follower (weights are omitted if they are both equal to 0).
infinite path for their respective dimension.
Each player's objective is to maximize the long run average of the payoffs that she receives (a.k.a. mean-payoff). 

In the adversarial Stackelberg setting, Player~0 (Leader) first announces how she will play then Player~1 (Follower) chooses one of his best-reponse to this strategy. Here, there are two choices for Player~0: $L$ or $R$. As Player~1 is assumed to be rational, Player~0 deduces that she must play $L$. Indeed, the best response of Player~1 is then to play $LL$ and the reward she obtains is $10$. This is better than playing $R$, for which the best response of Player~1 is $RL$, and the reward is $8$ instead of $10$. Note that if there are several possible best responses for Player~1, then we consider the worst-case: Player~0 has no control on the choice of best-responses by Player~1.


\subparagraph{{\bf Quantitative models and robustness}}
The study of the adversarial Stackelberg games with mean-payoff objectives has been started in~\cite{FGR20} with the concept of {\em adversarial Stackelberg value} ($\asvgen$ for short). $\asvgen$ is the best value that the leader can obtain by fixing her strategy and facing any rational response by the follower. As this setting is quantitative, it  naturally triggers questions about {\em robustness} that were left open in this first paper. 


Robustness is a {\em highly desirable} property of quantitative models: small changes in the quantities appearing in a model $M$ (e.g. rewards, probabilities, etc.) should have small impacts on the predictions made from $M$, see e.g.~\cite{BCGHHJKK14}.
Robustness is thus crucial because it accounts for modelling imprecision that are inherent in quantitative modelling and those imprecision may have important consequences. 
For instance, a reactive program synthesized from a model $M$ should provide acceptable performances even if it is executed in an environment that differ slightly w.r.t. the quantities modeled in $M$.

Some classes of models are robust. 
For instance, consider two-player {\em zero-sum} mean-payoff games where players have fully antagonistic objectives.
The \emph{value} of a two-player zero-sum mean-payoff $\mathcal{G}$ is the maximum mean-payoff that Player~0 can ensure against all strategies of Player~1.
A strategy $\sigma_0$ that enforces the optimal value $c$ in $\mathcal{G}$ is {\em robust} in the following sense. 
Let $\mathcal{G}^{\pm \delta}$ be the set of games obtained by increasing or decreasing the weights on the edges of $\mathcal{G}$ by at most $\delta$.
Then for all $\delta > 0$, and for all $\mathcal{H} \in \mathcal{G}^{\pm \delta}$, the strategy $\sigma_0$ ensures in $\mathcal{H}$ a mean-payoff of at least $c-\delta$ for Player~0 against any strategy of Player~1 (Theorem~\ref{robustZS}). So slight changes in the quantities appearing in the model have only a small impact on the worst-case value enforced by the strategy. 
\begin{comment}
For instance, the worst-case value in two player zero-sum mean-payoff games is {\em robust} in the following sense: if Player~0 has a strategy $\sigma_0$ to force a value $c$ against all the strategies of Player~1 in a game $G$, then for all $\delta >0$, for all games $H \in G^{\pm \delta}$ obtained from $G$ by keeping the underlying graph same but with weights that can be increased or decreased by upto $\delta$, then the worst-case optimal strategy $\sigma_0$ computed from $G$ has a worst-case value in $H$ which is guaranteed to be at least $c - \delta$ (see Theorem~\ref{robustZS}). 
\end{comment}

The situation is more complex and less satisfactory in {\em nonzero-sum} games. Strategies that enforce the $\asvgen$ proposed in~\cite{FGR20} may be {\em fragile}: slight differences in the weights of the game, or in the optimality of the response by Player~1, may lead to large differences in the value obtained by the strategy.

Let us illustrate those difficulties on our running example. The strategy of Player~0 that chooses $L$ in $v_0$ ensures her a payoff of $10$ which is the $\asvgen$.
Indeed, the unique best-response of Player~1 against $L$ is to play $LL$ from $v_1$. However, if the weights in $\mathcal{G}$ are changed by up to $\pm \delta=\pm 0.6$
then there is a game $\mathcal{H} \in \mathcal{G}^{\pm \delta}$ in which the weight on the self-loop over vertex $v_4$ changes to e.g. $9.55$, and the weight on the self-loop over $v_3$ changes to e.g. $9.45$, and the action $LR$ becomes better for Player~1.
So the adversarial Stackelberg value of $L$ in the new game $\mathcal{H}$ is now $0$ instead of $10$. Thus a slight change in the rewards for Player~1 (due to modelling imprecision for example) may have a dramatic effect on the value of the optimal strategy $L$ computed on the model $\mathcal{G}$ when evaluated in $\mathcal{H}$. 


\subparagraph{{\bf Contributions}}
To remedy to this situation, we provide a alternative notion of value that is better-suited to synthesize strategies that are robust against perturbations. We consider two types of perturbations. First, the strategies computed for this value are robust against {\em modeling imprecision}: if a strategy has been synthesized from a weighted game graph with weights that are possibly slightly wrong, the value that this strategy deliver is guaranteed to be close to what the model predicts. Second,  strategies computed for this value are robust against {\em sub-optimal responses}: small deviations from the best-response by the adversary have only limited effect on the value guaranteed by the strategy.

Our solution relies on relaxing the notion of best-responses of Player~1 \emph{in the original model $\mathcal{G}$}. More precisely, we define the $\epsilon$-adversarial Stackelberg  value ($\asv$, for short) as the value that Leader can enforce against all $\epsilon$-best responses of Follower. Obviously, this directly accounts for the second type of perturbations. But we show that, additionally, this accounts for the first type of perturbations: if a strategy $\sigma_0$ enforces an $\asv$ equal to $c$ then for all games $\mathcal{H} \in G^{\pm \frac{\epsilon}{2}}$, we have that $\sigma_0$ enforce a value larger than $c-\epsilon$ in $\mathcal{H}$ (Theorem~\ref{thm:combined-robustness} and Theorem~\ref{robustNZS}). 

We illustrate this by considering again the example of Figure~\ref{fig:robust-game-example}. 
Here, if we consider that the adversary can play $2\delta=1.2$-best responses
instead of best responses only, then the optimal strategy of Player~0 is now $R$ and it has a $\asv$ equal to $8$. This value is guaranteed to be robust for all games $\mathcal{H} \in \mathcal{G}^{\pm \delta}$ as $R$ is guaranteed to enforce a payoff that is larger than or equal to $8-\delta$ in all games in $\mathcal{G}^{\pm \delta}$.  
Stated otherwise, we use the notion of $\asv$ in the original game to find a strategy for Player~0 that she uses in the perturbed model while playing against a rational adversary.
Thus we show that in the event of modelling imprecision resulting in a perturbed model, the solution concept to be used is $\asv$ instead of $\asvgen$ since the former provides strategies that are robust to such perturbations.


\begin{figure}[t]
\centering
\begin{minipage}{.35\textwidth}
\centering
\scalebox{0.8}{
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.5cm,
                        semithick, squarednode/.style={rectangle, draw=blue!60, fill=blue!5, very thick, minimum size=7mm}, scale=.8]
      \tikzstyle{every state}=[fill=white,draw=black,text=black,minimum size=8mm]
    
      \node[squarednode]                                                 (A)              {$v_0$};
      \node[state, draw=red!60, fill=red!5]                              (B) [left of=A]  {$v_2$};
      \node[state, draw=red!60, fill=red!5]                              (C) [right of=A] {$v_1$};
      \node[draw=none, fill=none, minimum size=0cm, node distance = 1.2cm] (D) [above of=A] {$start$};
      \node[state, draw=red!60, fill=red!5]                              (E) [left of=B]  {$v_3$};
      \path (A) edge              node {} (B)
                edge              node {} (C)
            (B) edge [loop above] node {(1,1)} (B)
                edge              node {} (E)
            (C) edge [loop above] node {(0,1)} (C)
            (E) edge [loop above] node {(2,0)} (E)
            (D) edge [left] node {} (A);
    \end{tikzpicture}}
    \caption{Co-operative and adversarial followers in Stackelberg mean-payoff games}
    \label{fig:co-operative_vs_adversarial}
\end{minipage}
\quad
\begin{minipage}{.55\textwidth}
\centering
\scalebox{.8}{
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.4cm,
                        semithick, squarednode/.style={rectangle, draw=blue!60, fill=blue!5, very thick, minimum size=7mm}, scale=.8]
    
      \tikzstyle{every state}=[fill=white,draw=black,text=black,minimum size=8mm]
      \node[state, draw=red!60, fill=red!5]                              (A)                {$v_0$};
      \node[squarednode]                                                 (A_1) [right of=A] {$v_2$};
      \node[state, draw=red!60, fill=red!5]                              (B_1) [right of=A_1]  {$v_5$};
      \node[state, draw=red!60, fill=red!5]                              (C_1) [right of=B_1] {$v_6$};
      \node[squarednode]                                                 (A_2) [left of=A] {$v_1$};
      \node[state, draw=red!60, fill=red!5]                              (B_2) [left of=A_2]  {$v_3$};
      \node[state, draw=red!60, fill=red!5]                              (C_2) [left of=B_2] {$v_4$};
      \node[draw=none, fill=none, minimum size=0cm, node distance = 1.2cm] (D) [above of=A] {$start$};
      \path (A)   edge [, above ]          node {$R$}       (A_1)
                  edge [, above ]          node {$L$}       (A_2)
            (A_1) edge [, above ]          node {$RL$}      (B_1)
                  edge [bend right, below] node {$RR$}      (C_1)
            (A_2) edge [, above ]          node {$LL$}      (B_2)
                  edge [bend left]         node {$LR$}      (C_2)
            (B_1) edge [loop above]        node {$(8, 9)$}  (B_1)
            (C_1) edge [loop above]        node {$(4, 5)$}  (C_1)
            (B_2) edge [loop above]        node {$(10, 10)$} (B_2)
            (C_2) edge [loop above]        node {$(0, 9)$}  (C_2)
            (D)   edge [left]              node {}          (A);
    \end{tikzpicture}}
    \caption{A game in which the strategy of the leader that maximizes the adversarial Stackelberg is fragile while the strategy of the leader that maximizes the $\epsilon=1$-adversarial Stackelberg value is robust.\label{fig:robust-game-example}}
    
\end{minipage}
\end{figure}
\begin{comment}
\begin{table}[h]
\scalebox{0.85}{
\begin{tabular}{|c|c|c|c|c|}
\hline
 &
  \track{Robustness} &
  Threshold Problem &
  Computing ASV &
  Achievability \\ \hline
\begin{tabular}[c]{@{}c@{}}Adversarial \\ best responses \\ of the follower\end{tabular} &
    \begin{tabular}[c]{@{}c@{}}{ \textbf{\track{No}}} \\ \\ { \textbf{ \track{[\cref{fragile}]}}} \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}{ {\sf NP} \cite{FGR20}} \\ \\ { \textbf{Finite}} {\textbf{Memory}} \\ { \textbf{Strategy}} { \textbf{ [Thm \ref{LemFinMemWitnessASVNonEps}]}} 
  \\ \\
  {\track{\textbf{Memoryless}}} \\ {\track{\textbf{Strategy}}} 
  {\track{\textbf{[Cor \ref{cor:memoryless}]}}}
  \end{tabular} &
  \begin{tabular}[c]{@{}c@{}}{ Theory of Reals \cite{FGR20}} \end{tabular} &
  { No \cite{FGR20}} \\ \hline
\begin{tabular}[c]{@{}c@{}}Adversarial\\ $\epsilon$-best responses \\ of the follower\end{tabular} &
    \begin{tabular}[c]{@{}c@{}}{ \textbf{\track{Yes}}} \\ \\ { \textbf{ \track{[Thm \ref{robustNZS}]}}} \end{tabular} &
  { \textbf{\begin{tabular}[c]{@{}c@{}}{\sf \bf NP}\\ \\ Finite Memory \\ Strategy {[}Thm \ref{ThmNpForASV}{]}
  \\ \\
  {\track{\textbf{Memoryless}}} \\ {\track{\textbf{Strategy}}} 
  {\track{\textbf{ [Cor \ref{cor:memoryless}]}}} 
\end{tabular}}} &
  { \textbf{\begin{tabular}[c]{@{}c@{}}Theory of Reals\\  {[}Thm \ref{ThmComputeASV}{]} \\ \\ Solving LP \\ in {\sf EXPTime} \\ {[}Thm \ref{ExpTimeForComputeASV}{]} \end{tabular}}} &
  { \textbf{\begin{tabular}[c]{@{}c@{}}Yes {[}Thm \ref{ThmAchiev}{]} \\ \\ (Requires \\ Infinite  Memory\\  {[}Thm \ref{ThmExNeedInfMem}{]}) \end{tabular}}} \\ \hline
\end{tabular}}
% \begin{center}
    \caption{Summary of our results}
% \end{center}
\vspace{-.3cm}
\label{tab:results}
\end{table}
\end{comment}



In addition to proving the fragility of the original concept introduced in~\cite{FGR20} (\cref{fragile}) and the introduction of the new notion of value $\asv$ that is robust against modelling imprecision (\cref{robustNZS}), we provide algorithms to handle $\asv$.
First, we show how to decide the threshold problem for $\asv$ in nondeterministic polynomial time and that finite memory strategies suffice (\cref{ThmNpForASV}). Second, we provide an algorithm to compute $\asv$ when $\epsilon$ is fixed (\cref{ExpTimeForComputeASV}).
Third, we provide an algorithm that given a threshold value $c$, compute the largest possible $\epsilon$ that can be covered and such that $\asv > c$ (\cref{thm:ComputeEpsilon}). Those three results represent the core technical contributions of this paper and they are presented in Sect.~4 and Sect.~5.
Additionally, in Sect.~6, we provide results that concern the memory needed for players to play optimally, and complexity results for subcases (for example when Players are assumed to play memoryless).
Finally, we show that $\asv$ is always achievable (\cref{ThmAchiev}), which is in contrast to the case in \cite{FGR20} where the follower only plays best-responses.

\subparagraph{Related Works}
Stackelberg games on graphs have been first considered in \cite{FKL10}, where the authors study rational synthesis for $\omega$-regular objectives with co-operative followers.
In \cite{FGR20}, Stackelberg mean-payoff games in adversarial setting, and  Stackelberg discounted sum games in both adversarial and co-operative setting have been considered. 
However, as pointed out earlier, the model of \cite{FGR20} is not robust to perturbations.
In \cite{GS14}, mean-payoff Stackelberg games in the co-operative setting have been studied. 
In \cite{GS15}, the authors study the effects of limited memory on both Nash and Stackelberg (or leader) strategies in multi-player discounted sum games.
Incentive equilibrium over bi-matrix games and over mean-payoff games in a co-operative setting have been studied in \cite{GS18} and \cite{GSTDP16} respectively.
In \cite{KPV16}, adversarial rational synthesis for $\omega$-regular objectives have been studied.
In \cite{CFGR16}, precise complexity results for various $\omega$-regular objectives have been established for both adversarial and co-operative settings.
In \cite{CHJ06,BMR14}, secure Nash equilibrium has been studied, where each player first maximises her own payoff, and then minimises the payoff of the other player;
Player~0 and Player~1 are symmetric there unlike in Stackelberg games. For discounted sum objectives, in \cite{FGR20}, the gap problem has been studied.
Given rationals $c$ and $\delta$, a solution to the gap problem can decide if $\asvgen > c+\delta$ or $\asvgen < c-\delta$.
The threshold problem was left open in \cite{FGR20}, and is technically challenging.
We leave the case of analysing robustness for discounted sum objective
for future work.

A full version of this work with detailed proofs appears in \cite{BGR20}.

==> achievable.tex <==
\begin{conjecture}
For all mean-payoff games $\mathcal{G}$, for all vertices $v$ in $\mathcal{G}$ and for all $\epsilon > 0$ we have that $\asv(v)$ is achievable.
\end{conjecture}
\begin{proof}
Let $\asv(v) = c$.
Recall that $\asv(\sigma_0)(v) = \sup\limits_{\br(\sigma_0) \neq \varnothing}  \inf \limits_{\sigma_1 \in \br(\sigma_0)} \mpinf_0(\outv(\sigma_0,\sigma_1))$.
Then there exists a sequence of strategies $\sigma^0_0, \sigma^1_0, \dots$ such that $\lim \limits_{i \rightarrow \infty} \inf \limits_{\sigma_1 \in BR^{\epsilon}_1(\sigma^i_0)} \mpinf_0(\outv(\sigma_0,\sigma_1))=c$, and for all $i, j$ such that $j > i$, we have $\asv(\sigma_j)(v) \ge \asv(\sigma_i)(v)$.
W.l.o.g., we can assume that the memory used in strategy $\sigma_j$ is greater than the memory used in strategy $\sigma_i$ for $j > i$.
We use $\sigma_\infty$ to denote an infinite memory strategy of Player $0$.
If there exists an index $i \in \nat$ such that $\asv(\sigma_j)(v) = \asv(\sigma_i)(v)$ for all $j \ge i$ and for $j=\infty$, then $\sigma_i$ achieves $\asv(v)$.
Thus we consider the case where such an $i$ does not exist.

For every strategy $\sigma^i_0$ for $i \in \nat$, we have a sequence of plays $\pi^i_1, \pi^i_2, \dots$ such that $\lim \limits_{j \rightarrow \infty}\mpinf_1(\pi^i_j) = \sup \limits_{\sigma_1 \in \br(\sigma^i_0)} \mpinf_1(\sigma^i_0,\sigma_1)$.
W.l.o.g., assume that for every strategy $\sigma^i_0$, the plays $\pi^i_j$ for $j \in \nat$ end up in the same SCC $\mathbb{C}^i$, and for all $i,k \in \nat$, we have $\mathbb{C}^i=\mathbb{C}^j=\mathbb{C}$.

Let $d_i = \sup \limits_{\sigma_1 \in \br(\sigma^i_0)} \mpinf_1(\sigma^i_0,\sigma_1)$ for $i \in \nat \cup \{\infty\}$.
We have the following claim.
\begin{lemma}[conjecture] \label{lem:monotone}
The sequence ($d_i$)$_{i \in \nat \cup \{\infty\}}$ is monotonic.
\end{lemma}
\begin{proof}
Recall that the strategies $\sigma^1_0, \sigma^2_0, \dots$ use increasing amount of memory, that is, the memory needed by $\sigma^j_0$ is more than the memory used by $\sigma^i_0$ for $j > i$.
The values $d_0, d_1, \dots$ correspond to values that are obtained as a result of changing frequencies of the occurrences of the simple cycles in $\mathbb{C}$ in their corresponding plays.
Again, we can assume w.l.o.g. that these frequencies of the simple cycles in the SCC $\mathbb{C}$ change monotonically for $\sigma^0_0, \sigma^1_0, \dots$ for the plays that correspond to these values $d_0, d_1, \dots$, and hence the sequence ($d_i$)$_{i \in \nat \cup \{\infty\}}$ is monotonic.
\end{proof}

Now since the sequence ($d_i$) is monotonic, there can be two cases.
\begin{enumerate}
    \item The sequence ($d_i$)$_{i \in \nat}$ is monotonically non-decreasing
    \item The sequence ($d_i$)$_{i \in \nat}$ is monotonically decreasing
\end{enumerate}
We start with the first case; there can be two sub-cases.
\begin{enumerate}
\item[i] There exists an $i \in \nat$ such that for all $j \geqslant i$, and for $j=\infty$, we have that $d_j=d_i$.
Thus the sequence gets a ceiling.
Hence Player $1$ chooses the $\epsilon$-best-response that reduces the cost of Player $0$ the most, and thus $\asv(v)$ is achievable by Player $0$ as $\lim \limits{i \rightarrow \infty}$.
\item[ii] The sequence ($d_i$)$_{i \in \nat}$ is increasing.
Let $d = \lim \limits_{i \rightarrow \infty} d_i$, and $\pi$ be the corresponding play such that $\mpinf_1(\pi) = d$, and let $\pi_i$ be the play such that $\mpinf_1(\pi_i)=d_i$ for all $i \in \nat$.

Assume for contradiction that $\asv(v)$ is not achievable.
Then there exists $k \in \nat$ such that $\lim \limits_{i \rightarrow \infty} \asv(\sigma_i)(v) < \asv(\sigma_k)(v)$.
This implies that there exists a Player $1$ strategy $\sigma_\infty^1 \in \br(\sigma_\infty)$ such that $\mpinf_0(\outv(\sigma_\infty,\sigma_\infty^1)) = c' < c$.
Let $\pi'= \outv(\sigma_\infty,\sigma_\infty^1)$.
Consider the case $\inf(\pi') \subseteq S$.
Note that $\mpinf_1(\pi') = d'\ge d - \epsilon$, and let $\mpinf_0(\pi')=c'$.

If $d' < d$, then there exists an index $k$ such that $d_k > d'$, and by definition of $\sup$, we have that $\asv(\sigma_k)(v)=c''$ such that $c'< c'' \le c$.
Note that for all $v \in S$, we also have that $v$ is not $(c'', d_k)^\epsilon$-bad.
Now note that $d_k > d' > d_k -\epsilon$.
Hence, for every play $\pi'$ such that $\mpinf_1(\pi')=d'$, Player $1$ cannot ensure $\mpinf_0(\pi')=c' < c''$, and hence a contradiction.

Now consider the case where $d' = d$.
Recall that the corresponding play is $\pi$.
% Now we observe the relation between $\asv(\pi_k)$ and $\mpinf_0(\pi_k)$ to argue that $\asv(v)$ is achievable.
Note that for all $k \in \nat$, we have that $\mpinf_0(\pi_k) \ge \asv(\pi_k)$.
Since from Lemma \ref{lem:monotone}, we have that the sequence $(d_k)_{k \in \nat \cup {\infty}}$ is a monotone, we also have that the sequence $(\mpinf_0(\pi_k))_{k \in \nat \cup {\infty}}$ is a monotone.
Since $(\mpinf_0(\pi_k))_{k \in \nat \cup {\infty}}$ is a monotone, and $\mpinf_0(\pi_k) \ge \asv(v)$ for all $k \in \nat$, we have that $\asv(v)=\mpinf_0(\pi) \ge \asv(\sigma_k)(v)$ for all $k \in \nat$, and hence $\asv(v)$ is achievable.
Note that if there exists a $k \in \nat$ such that $\asv(v) < \asv(\sigma_k)(v)$, then there exists a $j > k$ such that $\asv(\sigma_j)(v) < \asv(\sigma_k)(v)$, a contradiction.

For $\inf(\pi') \not \subseteq S$, we have that Player $1$ could also deviate for every finite $k \in \nat$, and hence $\asv(v)$ is achievable.

% Now the $\asv(v)$ is not achievable by Player $0$ if there exists a $k \in \nat$ such that $\mpinf_0(\pi_k) > \mpinf_0(\pi)$, and for all $i, j \in \nat$, we have that $d_j > d_i$ if $j > i$.
% However, this is not possible since changing frequency of the simple cycles should change the values monotonically across both the dimensions.
\end{enumerate}
Now we consider the case where the sequence ($d_i$)$_{i \in \nat}$ is monotonically decreasing.
Again, in such a case, we only need to consider the case when $\lim \limits_{i \rightarrow \infty}$ since for $i \in \nat$, we have that $\asv(v)$ is achievable from the definition.
Let $d = \lim \limits_{i \rightarrow \infty} d_i$.
If $\asv(v)$ is not achievable, in such a case, we have that Player $1$ has a strategy $\sigma_1'$ such that $\mpinf_1(\lim \limits_{i \rightarrow \infty} \sigma_0^i, \sigma_1') > d-\epsilon$.
Let $\mpinf_1(\lim \limits_{i \rightarrow \infty} \sigma_0^i, \sigma_1') = d' =  d-\epsilon+\delta$, and $\mpinf_0(\lim \limits_{i \rightarrow \infty} \sigma_0^i, \sigma_1') = c'$.
In such a case, there exists a $k \in \nat$ such that $\mpinf_0(\pi_k)=c'$, and hence if $c'=\asv(v)$, it is achievable.
\end{proof}

==> conc.tex <==
In this work, we considered two-player nonzero-sum infinite duration mean-payoff Stackelberg games played on graph arenas. We also assumed that the follower is bounded rational, and hence would always choose an $\epsilon$-best-response to the leader's strategy.

\btrack{In \cite{FGR20}, the authors assume that the follower is fully rational, and thus will always play an adversarial best-response for a given strategy of the leader (when it exists).}
However, the assumption that the follower is fully rational may not always be realistic.
% , and thus we considered bounded rationality of the follower.

We considered the threshold problem, i.e, checking if $\asv > c$, and showed that the problem is in $\mathsf{NP}$, and it is at least as hard as the value problem in zero-sum mean-payoff games.
Additionally, we showed that if $\asv > c$, \track{we can construct a pseudopolynomial memory strategy for the leader to achieve this threshold.}
% We further show that the threshold problem is at least as hard as the value problem in zero-sum mean-payoff games whose precise complexity is a longstanding open problem.
We also showed that both $\asv$ and $\mathbf{ASV}$ remain unaffected when the leader is allowed to use only finite memory strategies.
\btrack{We gave an $\mathsf{EXPTime}$ algorithm to compute the $\asv$, and showed that the $\asv$ is always achievable, possibly with an infinite memory strategy, which is in contrast with the framework where the follower is perfectly rational \cite{FGR20}.}
\begin{comment}
We show that infinite memory is required for the leader to achieve the $\asv$. We also show that the follower may require infinite memory to play an $\epsilon$-best-response. 
Next we considered the threshold problem, i.e, checking if $\asv > c$, and showed that the problem is in $\mathsf{NP}$. Additionally, we show that if $\asv > c$, \track{we can construct a pseudopolynomial memory strategy for the leader to achieve this threshold.}
We also provided a relative hardness result showing that the threshold problem is hard for the value problem in zero-sum mean-payoff games whose precise complexity is a longstanding open problem.
We then considered the problem of computing the $\asv$, and showed that the $\asv$ can be expressed as a formula in the theory of reals with addition. Furthermore, we showed that this formula can be expressed as a set of exponentially many linear programs, which can be solved in $\mathsf{EXPTime}$ to compute the $\asv$.
We also consider the case when Player~$0$ is restricted to use only finite memory strategies.
This value is denoted by $\asv_{\sf FM}$.
We show that $\asv_{\sf FM} = \asv$.
Finally, we show that $\asv$ is always achievable.
\end{comment}

% For future work, we consider several short-term and long-term research directions.
Several problems related to the results presented here can be studied.
% Though we looked at the upper bounds of different problems, we have not yet looked at the hardness of problems that we studied here, for example, the threshold problem.
We conjecture that the threshold problem is at least as hard as deciding the existence of a winning strategy in zero-sum mean-payoff games in a bi-weighted game graph \cite{VCDHRR15} whose precise complexity is also an open problem.
% As a first step, 
We would like to study this relative hardness result.
Another interesting direction is to explore possible characterization of Stackelberg mean-payoff games where a finite memory strategy of Player~$0$ suffices to achieve the $\asv$.
This will allow us to get an estimate of how ``complex'' a game is in terms of the memory required by Player~$0$ in order to achieve the $\asv$.

Several extensions to this work are possible. Some of them are mentioned below.
\begin{enumerate}
    \item \textbf{Multiple followers} We studied Stackelberg mean-payoff games with one bounded rational follower. One natural extension to this work is to study games with multiple adversarial followers.
    % This would model how players would react in a more realistic situation.
    \item \textbf{Other Quantitative Objectives} 
    % In this work, we studied Stackelberg mean-payoff games where  each player has mean-payoff objectives. We can also extend this work to study
    Stackelberg games with adversarial follower can also be studied for the case of other quantitative objectives such as discounted sum or quantitative reachability.
    One can even consider extensions with combinations of various quantitative objectives.
    \item \textbf{Other Solution Concepts} The main solution concept that is focused on in this work is Nash Equilibrium. Subgame perfect equilibrium is another solution concept that can be studied in both the co-operative as well as the adversarial setting.
    \item \textbf{Multiple leaders} It would be interesting to explore the scenario where there are several leaders,
    % who are in an equilibrium (such as Nash), 
    and each leader has several followers. 
    One can consider lexicographically ordered objectives, for example, that the leaders are rational yet adversarial to each other, and thus, would try to maximize their own payoff first, and then minimize the payoff of the other leaders. 
\end{enumerate}

==> fin_memory_example.tex <==
% \begin{figure}
%     \centering
%     \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3.8cm,
%                         semithick, squarednode/.style={rectangle, draw=blue!60, fill=blue!5, very thick, minimum size=15mm}]
%       \tikzstyle{every state}=[fill=white,draw=black,text=black,minimum size=2cm]
    
%       \node[squarednode]   (A)                    {$v_0$};
%       \node[state, draw=red!60, fill=red!5]         (B) [left of=A] {$v_1$};
%       \node[state, draw=red!60, fill=red!5]         (C) [right of=A] {$v_2$};
%       \node[draw=none, fill=none, minimum size=0cm, node distance = 2cm]         (D) [above of=A] {$start$};
%       \path (A) edge [bend left, below] node {(1,1)} (B)
%                 edge              node {(0,1)} (C)
%             (B) edge [loop above] node {(0,2)} (B)
%                 edge [bend left, above] node {(1,1)} (A)
%             (C) edge [loop above] node {(0,1)} (C)
%             (D) edge [left] node {} (A);
%     \end{tikzpicture}
%     \caption{An example in which a finite memory strategy for Player $0$ suffices to achieve $\asv(v_0)$.}
%     \label{fig:finite_strategy_response}
% \end{figure}
\sgcomment{Move this to appendix.}
\begin{theorem}
\label{ThmExNeedFinMem}
There exists a mean-payoff game $\mathcal{G}$, a vertex $v$ in $\mathcal{G}$, and an $\epsilon > 0$ such that a finite memory strategy of Player $0$ suffices to achieve $\asv(v)$.
\end{theorem}

==> finite_epsilon_strategy.tex <==
\begin{theorem}
\label{ThmP1NeedInfMem}
It is not true that for all mean-payoff games $\mathcal{G}$, for all Player $0$ strategies $\sigma_0$, and for all $\epsilon > 0$, there exists a finite memory strategy $\sigma_1$ of Player $1$ such that $\sigma_1 \in \br(\sigma_0)$.
\end{theorem}
\begin{figure}
    \centering
    \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3.8cm,
                        semithick, squarednode/.style={rectangle, draw=blue!60, fill=blue!5, very thick, minimum size=15mm}]
      \tikzstyle{every state}=[fill=white,draw=black,text=black,minimum size=2cm]
    
      \node[state, draw=red!60, fill=red!5]   (A)                    {$v_0$};
      \node[squarednode]         (B) [left of=A] {$v_1$};
      \node[state, draw=red!60, fill=red!5]         (C) [right of=A] {$v_2$};
      \node[draw=none, fill=none, minimum size=0cm, node distance = 2cm]         (D) [below of=A] {$start$};
      \path (A) edge [bend left, below] node {(0,0)} (B)
                edge              node {(0,0)} (C)
                edge [loop above] node {(0,3)} (A)
            (B) edge [loop above] node {(3,0)} (B)
                edge [bend left, above] node {(0,0)} (A)
            (C) edge [loop above] node {(1,0)} (C)
            (D) edge [left] node {} (A);
    \end{tikzpicture}
    \caption{No $\epsilon$-optimal finite memory response of Player $1$ to a strategy $\sigma_0$ of Player $0$}
    \label{fig:no_optimal_response}
\end{figure}
\begin{proof}
Consider the example in Figure \ref{fig:no_optimal_response}.
Consider the following strategy $\sigma_0$ of Player $0$.
Player $0$ loops over $v_0$ $i$ times, and then sends the token to $v_1$.
Player $1$ loops over $v_1$ $k$ times, and then sends the token to $v_0$.
If $k \geqslant i$, then Player $0$ increases $i$ by $1$, and repeats the above, otherwise sends the token to $v_2$.
Clearly for all $\epsilon \leqslant 1.5$, no finite memory strategy only is an $\epsilon$-best-response to $\sigma_0$.
\end{proof}

==> hardnessThreshold.tex <==

We show that the threshold problem is at least as hard as the value problem in the zero-sum mean-payoff games 
which is known to be in {\sf NP $\cap$ coNP}, and whose precise complexity is not known \cite{ZP96}.
% A small description of zero-sum mean-payoff games is provided in \textbf{\cref{sec:zero-sum}}.
\begin{comment}
The zero-sum mean-payoff game is played between two players, Player~0 and Player~1, for an infinite duration and on a finite (single) weighted arena $\mathcal{A} = (V,E, \zug{V_0,V_1}, w)$, where $V$ is a set of vertices partitioned into $V_0$ and $V_1$ belonging to Player~0 and Player~1 respectively, $E$ is a set of edges, and $w: E \rightarrow \mathbb{Q}$ assigns a rational weight to the edges of $\mathcal{A}$.
We denote the zero-sum mean-payoff game by $\mathcal{G}_0 = (\mathcal{A}, \mpgen)$.
Initially, a token is put on some vertex of $\mathcal{G}_0$. At each step of the play, the player controlling the vertex where the token is present chooses an outgoing edge and moves the token along the edge to the next vertex. Players interact in this way an infinite number of times and a play $\pi$ of the game is simply an infinite path traversed by the token.
At each step, the objective of Player~0 is to choose an outgoing edges from the vertices she owns in a way so as to maximise the $\liminf$ of the mean of the play $\pi$, denoted $\mathbf{\underline{MP}}(\pi)$, while the objective of Player~1 is the opposite.
Given a rational $c$, the \emph{value} problem in the zero-sum mean-payoff game is to decide whether Player~0 has a strategy to get a mean-payoff greater than $c$ against all possible strategies of Player~1.
Zero-sum mean-payoff games are determined, and optimal memoryless strategies are known to exist for both players.
\end{comment}

% We now state the following hardness result.
\begin{theorem} \label{ThmHardnessThreshold}
For all mean-payoff games $\mathcal{G}$, for all vertices $v$ in $\mathcal{G}$, for all $\epsilon > 0$, and for all rationals $c$, the problem of deciding if $\asv(v) > c$ or $\asvgen(v) > c$ is at least as hard as solving the value problem in zero-sum mean-payoff games.
\end{theorem}
The proof of this theorem appears in \cref{app:ThmHardnessThreshold}.



==> listOfSymbols.tex <==
\chapter*{List of Symbols}
\begin{longtable}{cp{0.6\textwidth}}
    $\mathbb{R}$ & Set of real numbers \\
    $\mathbb{R}^+$ & Set of positive real numbers \\
    $\mathbb{Q}$ & Set of rational numbers \\
    $\mathbb{Q}^+$ & Set of positive rational numbers \\
    $\mathbb{Q}^d$ & $d$-dimensional vector of rational numbers \\
    $\mathbb{Z}$ & Set of integers \\
    $\mathbb{N}$ & Set of natural numbers \\
    $\epsilon$ & Epsilon \\
    $\asvgen$ & Adversarial Stackelberg Value\\
    $\asvgen_\mathbf{FM}$ & Adversarial Stackelberg Value when leader is restricted to playing finite memory strategies \\
    $\asv$ & Epsilon-optimal Adversarial Stackelberg Value \\
    $\asv_\mathbf{FM}$ & Epsilon-optimal Adversarial Stackelberg Value when leader is restricted to playing finite memory strategies \\
    $\mathbf{NP}$-Time & Non-Deterministic Polynomial Time \\
    $\mathbf{EXP}$-Time & Exponential Time \\
    $\mathcal{A}$ & Arena \\
    $V$ & Set of Vertices \\
    $E$ & Set of Edges \\
    $w_i$ & Weight function of Player~i \\
    $\pi$ & Play in the arena \\
    $\mathcal{G}$ & Mean-payoff game \\
    $\mathbf{Plays}_\mathcal{A}$ & Set of Plays in arena $\mathcal{A}$ \\
    $\mathbf{Hist}_\mathcal{A}$ & Set of Histories in arena $\mathcal{A}$ \\
    $\mpinf_i$ & Mean-payoff function of Player~i \\
    $\mathbf{Out}_h$ & Outcome of a game with history $h$ \\
    $\sigma_i$ & Strategy of Player~i \\
    $\Sigma_i$ & Set of strategies of Player~i \\
    $\overline{\sigma}$ & Strategy profile \\
    $\mathbf{BR}_i$ & Best response of Player~i \\
    $\mathbf{BR}^{\epsilon}_i$ & Epsilon-optimal best response of Player~i \\
    $\mathsf{CH}$ & Convex Hull \\
    $\mathsf{SCC}$ & Strongly Connected Component \\
\end{longtable}
